Data-driven stochastic Lie transport modelling of the 2D Euler equations

In this paper, we propose and assess several stochastic parametrizations for data-driven modelling of the two-dimensional Euler equations using coarse-grid SPDEs. The framework of Stochastic Advection by Lie Transport (SALT) [Cotter et al., 2019] is employed to define a stochastic forcing that is decomposed in terms of a deterministic basis (empirical orthogonal functions, EOFs) multiplied by temporal traces, here regarded as stochastic processes. The EOFs are obtained from a fine-grid data set and are defined in conjunction with corresponding deterministic time series. We construct stochastic processes that mimic properties of the measured time series. In particular, the processes are defined such that the underlying probability density functions (pdfs) or the estimated correlation time of the time series are retained. These stochastic models are compared to stochastic forcing based on Gaussian noise, which does not use any information of the time series. We perform uncertainty quantification tests and compare stochastic ensembles in terms of mean and spread. Reduced uncertainty is observed for the developed models. On short timescales, such as those used for data assimilation [Cotter et al., 2020], the stochastic models show a reduced ensemble mean error and a reduced spread. Particularly, using estimated pdfs yields stochastic ensembles which rarely fail to capture the reference solution on small time scales, whereas introducing correlation into the stochastic models improves the quality of the coarse-grid predictions with respect to Gaussian noise.

==> 2022-06-22 ArXiv/introduction_idea_unused.tex <==

\begin{itemize}
\item \textbf{What?} Stochastic forcing of a dynamical system based on different underlying probability distributions and/or statistical properties of measurements.
\item \textbf{Why?} Not all information of the measurements has been used - the EOF algorithm provides us with more data than just the $\boldsymbol \xi_i$; we also have access to the corresponding time series. With little effort we can investigate how additional information of the measurements influences the stochastically forced system. In essence, we investigate the assumption of Gaussian noise in the SALT approach.
\item \textbf{How?} The additional information of the system/simulation is obtained by analyzing the available measurements. In this case it provides us with time series corresponding to eigenfunctions of the data. The time series are represented as either a randomly drawn signal from a histogram, or an autoregressive time series.
\item \textbf{What next?} This technique can be applied to other models as well, such as the shallow water equations or Rayleigh-B\'enard convection, or provide an additional technique in data assimilation to generate an ensemble of solutions with reduced uncertainty.
\end{itemize}

Introduction idea:
\begin{itemize}
    \item \textit{Challenge in geophysical and observational sciences: resolving small scales. Solution: use of stochasticity.} 
    \item \textit{Inclusion of data to account for uncertainty and unresolved scales. How: data-driven modeling and stochasticity. }
    \item \textit{Mention SALT and the inclusion of EOFs}
    \item \textit{(?) Related topics: data assimilation as a tool to reduce uncertainty `on the fly', LES as a means to accurately simulate flows on coarse grids.}
    \item \textit{Describe the of SALT application to the Euler problem. Mention the assumption of Gaussian noise, and the availability of additional data (time series) which prompts us to try to use this information.}
    \item \textit{State the goal of the paper and what the main findings and their implications are.}
    Goal: provide an accurate and precise ensemble of forecasts using information obtained from the measurements. \\
\end{itemize}


==> 2022-06-22 ArXiv/preamble.tex <==
\usepackage[utf8]{inputenc}
\usepackage[english]{babel} % English language/hyphenation
\usepackage{amsmath,amssymb,amsthm} % Math packages
\usepackage[margin=2cm]{geometry}
\usepackage{upgreek}
\usepackage{esint}
\usepackage[colorlinks]{hyperref}
\usepackage{todonotes}
\usepackage{enumerate}
\usepackage{framed}
\usepackage{pgfplots}
\usepackage{float}
\usepackage{tikz,tikz-cd}
\usepackage[all]{xy}
\usepackage{authblk}
\usepackage{caption}
\usepackage{subcaption}

==> 2022-06-22 ArXiv/previous_notes.tex <==
\appendix
\section{Previous notes}

\subsection{Governing equations}
The domain considered here is the two-dimensional unit square, denoted by $\mathcal{D}$.
\paragraph{Deterministic equations.} \begin{align}
    \partial_t \omega + \left(\mathbf{u}\cdot\nabla\right)\omega &=Q-r\omega, %\label{eq:hyperboliceqn}\\
    \mathbf{u}&=\nabla^\perp \psi, %\label{eq:gradperpeqn}\\
    \Delta \psi &= \omega, %\label{eq:poissoneqn}
\end{align}
where the forcing $Q$ is chosen as \begin{equation}
    Q(x,y) = \alpha\sin\left(\beta\pi x\right), \hspace{3mm} (x,y)\in\mathcal{D}.
    \label{eq: definition Q}
\end{equation}
A slip boundary is considered by applying \begin{equation}
    \psi|_{\partial\mathcal{D}}=0.
    %\label{eq:BC}
\end{equation}
Throughout the rest of this study, the values for $\alpha$ and $\beta$ are chosen to be $0.1$ and $8$, respectively. The damping parameter $r$ is set to $0.01$. The system given by \eqref{eq:hyperboliceqn}-\eqref{eq:poissoneqn} defines the evolution of the fluid, which is completely determined by the evolution of the vorticity. For this reason, the two-dimensional Euler equation describe vortex dynamics \cite{zeitlin2018geophysical}.

\paragraph{Stochastic equations.}
The equations are made stochastic by introducing stochastic forcing term based on the eigenvectors of the velocity-velocity correlation tensor. These eigenvectors are denoted by $\boldsymbol \xi_i$ and, by assuming that $\mathbf{u}$ is divergence-free, it can be shown that $\boldsymbol \xi_i$ are also divergence-free. Thus, each $\boldsymbol \xi_i$ can be expressed using a potential function $\zeta_i$ via \begin{equation}
    \boldsymbol \xi_i = \nabla^\perp \zeta_i.
    \label{eq:xiGradperp}
\end{equation}
The stochastic term is then introduced to advecting velocity by using the identity \begin{equation}
   \mathbf{u}(t)\text{d}t + \sum_i \boldsymbol\xi_i \circ \text{d}W_t^i = \nabla^\perp \psi(t)\text{d}t + \sum_i \nabla^\perp\zeta_i\circ\text{d}W_t^i.
   \label{eq:stocheqn}
\end{equation}

\paragraph{Numerical implementation.} A full description of the numerical implementation can be found in \cite{cotter2019numerically}, of which only the key details are included here for completeness.\\
A finite element method is employed to solve the system of equations \eqref{eq:hyperboliceqn}, \eqref{eq:gradperpeqn}, and \eqref{eq:poissoneqn}. The Poisson equation for the streamfunction is discretized using a continuous Galerkin scheme, whereas the vorticity equation \eqref{eq:hyperboliceqn} is discretized using a discontinuous Galerkin scheme. The space of discontinuous test functions guarantees numerical conservation of energy in the absence of source terms \cite{bernsen2006dis}. \\
Numerical time integration is performed by applying a third-order strong stability preserving Runge-Kutta (SSPRK3) method. Given a system $q_t = L(q)$, this method reads \begin{equation}
    \begin{aligned}
        q^{(1)} &= q^n + \Delta t L(q^n), \\
        q^{(2)} & = \frac{3}{4}q^{n} + \frac{1}{4}\left[ q^{(1)} + \Delta t L\left(q^{(1)}\right) \right], \\
        q^{n+1} & = \frac{1}{3}q^{n} + \frac{2}{3}\left[ q^{(2)} + \Delta t L\left( q^{(2)}\right) \right].
    \end{aligned}
    \label{eq:SSPRK3}
\end{equation}
Here the superscripts $n$ and $n+1$ denote the $n^\mathrm{th}$ and the ensuing time step, respectively. The internal stages of the Runge-Kutta algorithm are denoted by the superscripts $(1)$ and $(2)$. The time step size is given by $\Delta t$. The time integration scheme for a Stratonovich SPDE is similar. The system given by \begin{equation}
    \text{d}q(t) = L(q(t))\text{d}t + \sum_{i=1}^m G^i(q(t))\circ\text{d}W_t^i
\end{equation}
is integrated via 
\begin{equation}
    \begin{aligned}
        q^{(1)} &= q^n + \Delta t L(q^n) + \sum_{i=1}^n G^i(q^n)\Delta W^i, \\
        q^{(2)} & = \frac{3}{4}q^{n} + \frac{1}{4}\left[ q^{(1)} + \Delta t L\left(q^{(1)}\right) + \sum_{i=1}^n G^i\left(q^{(1)}\right)\Delta W^i \right], \\
        q^{n+1} & = \frac{1}{3}q^{n} + \frac{2}{3}\left[ q^{(2)} + \Delta t L\left( q^{(2)}\right) + \sum_{i=1}^n G^i\left(q^{(2)}\right)\Delta W^i \right].
    \end{aligned}
\end{equation}
Here $\Delta W^i$ denote random samples drawn from a standard normal distribution and multiplied by $\Delta t$.

\paragraph{Deterministic numerical simulation setup.} The deterministic numerical simulation as presented in \cite{cotter2019numerically} is used to generate the EOFs and corresponding time series. The system \eqref{eq:hyperboliceqn}-\eqref{eq:BC} are solved on a grid consisting of $512^2$ computational cells, which will be referred to as the fine grid. A time step size of $\Delta t=0.0025$ is adopted to ensure that a CFL number of $1/3$ is not exceeded. The initial condition of the simulation is described by the vorticity profile \begin{equation}
    \omega = \sin(8\pi x)\sin(8\pi y) + 0.4\cos(6\pi x)\cos(6\pi x) + 0.3\cos(10\pi x)\cos(4\pi y) + 0.02\sin(2\pi y) + 0.02\sin(2\pi x),
\end{equation}
from which the system will reach an equilibrium state after a spin-up time of 100 time units. 


\paragraph{Stochastic numerical simulation setup.} The stochastic numerical simulations are performed on a grid consisting of $64^2$ computational cells, which will be referred to as the coarse grid. A time step size $\Delta t=0.01$ is adopted for each simulation, in accordance with \cite{cotter2019numerically}. The initial conditions are given by the injected fine solution at $t=100$ (after the spin-up time). The fine vorticity is injected on the coarse grid, after which the corresponding streamfunction and velocity fields are calculated.

\paragraph{Perturbation of the initial conditions.} done to see how long the perturbed DNS takes to diverge from the `true' DNS. This gives us a maximum prediction horizon.

\subsection{Data acquisition and processing}
\paragraph{Lagrangian trajectory estimation.} The difference between the Lagrangian trajectories on the fine grid solution and on the filtered fine grid solution provide the measurements that are used in the EOF algorithm. In order to compare the trajectories for the different solutions, we define a fine grid time step $\Delta t_f$ and a coarse grid time step $\Delta t_c = k\Delta t_f$, where $k$ is some integer. Given a fine grid solution $\mathbf{u}^n$ at time $t^n = n\Delta t_c$, the Lagrangian trajectories starting from coordinates $(x_0,y_0)$ are acquired through the following steps.
\begin{itemize}
    \item The solution $\mathbf{u^n}$ is filtered to so that $\bar{\mathbf{u}}^n$ is obtained. The Lagrangian trajectory for the filtered fine grid is estimated via $\Delta t_c \bar{\mathbf{u}}(x_0,y_0)^n$.
    \item An estimate of the true Lagrangian trajectory is found by integrating the movement of a Lagrangian particle over time. That is, we define $(x_{i+1},y_{i+1}) = (x_i,y_i) + \Delta t_f \mathbf{u}(x_i,y_i)$ and apply this step for each of the $k$ fine grid time steps starting from $t^n$. Linear interpolation is applied when the intermediate position of the particle does not coincide with a grid point.
    \item The Lagrangian trajectory corresponding to the filtered solution is subtracted from the estimate of the true trajectory to obtain a distance that `belongs' to the position $(x_0,y_0)$ and time $t^n$.
\end{itemize}
At each coarse grid time step, the initial positions for the particles are chosen as the coarse grid points. The fine grid solution is filtered by applying the Helmholtz operator to the streamfunction $\psi$, i.e., the equation \begin{equation}
    (I-c\Delta)\bar{\psi} = \psi
\end{equation}
is solved for the filtered streamfunction $\bar{\psi}$. Since the coarse grid size consists of 64 cells in each spatial direction, $c$ is chosen equal to $1/64^2$ so that the filtered solution only contains frequencies that are resolvable on the coarse grid.

\paragraph{EOF algorithm and time series computation.} The EOF algorithm decomposes a signal $a(x,t)$ into a time-mean $\xi_0(x)$ and a sum of time series $a_i(t)$ multiplied by eigenfunctions (EOF modes, or EOFs) $\xi_i(x)$ according to \begin{equation}
    a(x,t) = \xi_0(x) + \sum_{i=1}^N a_i(t)\xi_i(x).
\end{equation}
The EOF modes are orthonormal, that is, $\langle \xi_i, \xi_j \rangle = \delta_{ij}$ where $\langle\cdot,\cdot\rangle$ denotes the inner product and $\delta_{ij}$ denotes the Kronecker delta. Due to the orthonormality, the coefficients $a_i(t)$ are readily obtained by taking the inner product of the de-trended measurements with the corresponding EOF mode, \begin{equation}
    a_i(t) = \langle a(x,t)-\xi_0(x), \xi_i(x) \rangle.
\end{equation}

\paragraph{Probability density estimation.} Central to the histogram noise is the assumption that the measured difference in Lagrangian trajectories can be characterized by an underlying probability density. An estimated probability density can then be obtained by constructing a histogram, based on the measurements. The histogram is a statistical estimator and therefore its quality is described by the bias and its robustness under changes of measurements by the variance. A trade-off occurs between these two values. Given a set of measurements, an unbiased histogram can be produced by letting each histogram bin contain only a single measurement, but such an estimator is prone to large changes as more measurements are added. On the other hand, a very robust estimator is obtained by constructing a histogram where all measurements fall within a single bin, although the bias of this histogram would be significant.\\
The number of bins in histogram is of importance, since histograms are determined entirely by the input data and the number of bins. The number of bins adopted here follows from the results presented in \cite{scott2015} and is based on minimizing the asymptotic integrated mean squared error (MSE). The MSE is defined as the sum of the variance and the square of the bias of the histogram. A lower bound for the number of bins is found by minimizing the asymptotic integrated MSE and is given by
 \begin{equation}
\text{Number of bins}\geq \sqrt[3]{2N_M},
\end{equation}
where $N_M$ denotes the number of measurements.

\subsubsection{Random noise generation}
Random numbers are generated using the random sampling package from the NumPy package for Python.
\paragraph{Gaussian noise.} Gaussian noise is generated by sampling from a standard normal distribution and subsequently multiplying by the square root of the time step ($\sqrt{\Delta t}$). The resulting samples are normally distributed with mean zero and variance $\Delta t$.
\paragraph{Histogram noise.}
The histograms are treated as discrete probability distributions. A single bin represents an event, where the height of the bin denotes the probability of that event taking place and the average of the bin edges determine the event value. Samples are drawn from the estimated distribution by applying inverse transform sampling.

\paragraph{Correlated noise.} An Ornstein-Uhlenbeck process is used to generate time-correlated noise. The process is given by the stochastic differential equation \begin{equation}
    \text{d}U(t) = -U(t)\frac{\text{d}t}{T} + \left(\frac{2\sigma^2}{T}\right)^{1/2} \text{d}W(t),
\end{equation}
where $T$ is a (positive) time scale, $\sigma$ is a constant and the initial condition $U(0)\sim\mathcal{N}(0,\sigma^2)$. The notation used here follows from \cite{pope2001}. A discrete form of this equation is given by the autoregressive (AR) model of order 1, \begin{equation}
    \begin{aligned}
        U_i &= U_{i-1} + \text{d}U_i, \\
        \text{d}U_i &= -U_{i-1}\frac{\Delta t}{T} + \left(\frac{2\sigma^2}{T}\right)^{1/2}r_i,
    \end{aligned}
\end{equation}
where $r_i\sim \mathcal{N}(0,\Delta t)$. The value of $T$ is chosen as the decorrelation time of the time series of the EOF modes. The parameter $\sigma$ is set equal to $\sqrt{T/2}$, so that the process reduces to Gaussian noise with variance $\Delta t$ when the decorrelation time is a single time step.\\
The decorrelation time is mode-dependent and is defined as the time at which the autocorrelation attains a nonpositive value for the first time. This way, the decorrelation time measured from the time series of the EOF modes and those of the generated time series using the OU process are similar.



\subsection{Results}
\paragraph{DNS sensitivity study.} Every coarse numerical solution can be regarded as a filtered fine solution. This is not a one-to-one relation, in fact, a filtered solution is invariant under perturbations of the fine solution as long as the perturbed lengthscales are smaller than the coarse grid size. Thus, given a coarse solution one can not know the fine grid solution that corresponds to the former. \\
The initial conditions of the fine simulation are altered by perturbing frequencies that can not be resolved on the coarse grid. By identifying a time at which the perturbed fine simulation results diverge, one identifies the time after which the coarse prediction can no longer be sensibly compared to the DNS result. The idea behind this is that the fine solutions do not correspond to the same filtered (coarse) solution after the fine solutions have diverged.

\paragraph{Temporal correlation of the flow.} To estimate the time scales present in the numerical solution, we compute the inner product of the velocity field at different times. The value \begin{equation}
    \frac{\langle \mathbf{u}(t_i), \mathbf{u}(t_j) \rangle}{\langle\mathbf{u}(t_i), \mathbf{u}(t_i) \rangle} = \frac{\int_\Omega\! \mathbf{u}(t_i) \cdot \mathbf{u}(t_j) \,\text{d}\Omega}{\int_\Omega \! \|\mathbf{u}(t_i)\|^2\text{d}\Omega}
\end{equation}
can be thought of as the similarity between to velocity fields $\mathbf{u}(t_i)$ and $\mathbf{u}(t_j)$. Applying this to the velocity field obtained from the truth and the filtered truth yields an indication of correlation time of the measurements.


\paragraph{Flow measures.}
We can describe the following things (based on the reference paper):\begin{itemize}
    \item Uncertainty quantification plots comparing the truth with the ensemble one standard deviation about the ensemble mean, using point values. We can compare the truth (coarse-grained fine solution), the coarse solution without additional modelling, and the coarse solution with stochasticity. (The 4x4 observation grid is used for data assimilation.) This is useful for comparing the results using a certain type of noise with the true solution. Additionally, plotting the results of multiple types of noise in one plot can be used for comparison between the methods.
    \item The relative $L^2$ distance between the SPDE ensemble and the coarse-grained truth. This quantity is given by \begin{equation}
        d\left(\left\{\hat{q}^i, i=1,\ldots,N_p\right\}\right) = \min_{i\in\{1,\ldots,N_p\}} \frac{\|\omega(t)-\hat{q}^i(t)\|_{L^2(\mathcal{D})}}{\|\omega(t)\|_{L^2(\mathcal{D})}},
    \end{equation}
    which describes the $L^2$ distance of the `best' particle at a given time. (Which particle is the `best' particle can change over time.) This is useful for comparing the results using different types of noise with each other.
\end{itemize}

\paragraph{Measures for predictive capabilities.} Ideas taken from \cite{leutbecher2009diagnosis}, \cite{arnold2013stochastic}, \cite{wilks2011statistical}
\begin{itemize}
    \item Short-term forecasting scale? (see L96 Palmer paper)
    \item rms error - rms spread plots? These plots provide a check for statistical consistency by verifying the relation \begin{equation}
        \frac{M}{M-1}\text{estimate ensemble variance} = \frac{M}{M+1}\text{squared ensemble mean error},
    \end{equation}
    see \cite{arnold2013stochastic}.
\end{itemize}



==> 2022-06-22 ArXiv/unused.tex <==

\iffalse
\subsection{\label{sec:longtime} Long-time statistics}
In order to understand the long-time effects of the different types of stochastic forcing on the solution, a set of time-averaged quantities are studied. The averages are obtained by sampling the numerical solution at every time unit after the spin-up time, for a total of 365 time units. A single realization is considered for each type of stochastic forcing.\\
\textbf{\textit{Remove figure b}}

\textit{Perhaps something like pdfs of the vorticity at certain points in the domain could be interesting as well?}

\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures_general/average_vorticity_spectra.eps}
    \caption{Average energy spectra of cross-sections of the vorticity field in $x$-direction.}
    \label{fig:RMSRME_filtered_DNS}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures_general/average_fluctuation_spectra.eps}
    \caption{Average energy spectra of cross-sections of the vorticity fluctuation field in $x$-direction.}
    \label{fig:RMSRME_coarse_with_xis}
    \end{subfigure}
    \caption{Test caption}
\end{figure}
\fi

==> introduction_idea_unused.tex <==

\begin{itemize}
\item \textbf{What?} Stochastic forcing of a dynamical system based on different underlying probability distributions and/or statistical properties of measurements.
\item \textbf{Why?} Not all information of the measurements has been used - the EOF algorithm provides us with more data than just the $\boldsymbol \xi_i$; we also have access to the corresponding time series. With little effort we can investigate how additional information of the measurements influences the stochastically forced system. In essence, we investigate the assumption of Gaussian noise in the SALT approach.
\item \textbf{How?} The additional information of the system/simulation is obtained by analyzing the available measurements. In this case it provides us with time series corresponding to eigenfunctions of the data. The time series are represented as either a randomly drawn signal from a histogram, or an autoregressive time series.
\item \textbf{What next?} This technique can be applied to other models as well, such as the shallow water equations or Rayleigh-B\'enard convection, or provide an additional technique in data assimilation to generate an ensemble of solutions with reduced uncertainty.
\end{itemize}

Introduction idea:
\begin{itemize}
    \item \textit{Challenge in geophysical and observational sciences: resolving small scales. Solution: use of stochasticity.} 
    \item \textit{Inclusion of data to account for uncertainty and unresolved scales. How: data-driven modeling and stochasticity. }
    \item \textit{Mention SALT and the inclusion of EOFs}
    \item \textit{(?) Related topics: data assimilation as a tool to reduce uncertainty `on the fly', LES as a means to accurately simulate flows on coarse grids.}
    \item \textit{Describe the of SALT application to the Euler problem. Mention the assumption of Gaussian noise, and the availability of additional data (time series) which prompts us to try to use this information.}
    \item \textit{State the goal of the paper and what the main findings and their implications are.}
    Goal: provide an accurate and precise ensemble of forecasts using information obtained from the measurements. \\
\end{itemize}


==> previous_notes.tex <==
\appendix
\section{Previous notes}

\subsection{Governing equations}
The domain considered here is the two-dimensional unit square, denoted by $\mathcal{D}$.
\paragraph{Deterministic equations.} \begin{align}
    \partial_t \omega + \left(\mathbf{u}\cdot\nabla\right)\omega &=Q-r\omega, %\label{eq:hyperboliceqn}\\
    \mathbf{u}&=\nabla^\perp \psi, %\label{eq:gradperpeqn}\\
    \Delta \psi &= \omega, %\label{eq:poissoneqn}
\end{align}
where the forcing $Q$ is chosen as \begin{equation}
    Q(x,y) = \alpha\sin\left(\beta\pi x\right), \hspace{3mm} (x,y)\in\mathcal{D}.
    \label{eq: definition Q}
\end{equation}
A slip boundary is considered by applying \begin{equation}
    \psi|_{\partial\mathcal{D}}=0.
    %\label{eq:BC}
\end{equation}
Throughout the rest of this study, the values for $\alpha$ and $\beta$ are chosen to be $0.1$ and $8$, respectively. The damping parameter $r$ is set to $0.01$. The system given by \eqref{eq:hyperboliceqn}-\eqref{eq:poissoneqn} defines the evolution of the fluid, which is completely determined by the evolution of the vorticity. For this reason, the two-dimensional Euler equation describe vortex dynamics \cite{zeitlin2018geophysical}.

\paragraph{Stochastic equations.}
The equations are made stochastic by introducing stochastic forcing term based on the eigenvectors of the velocity-velocity correlation tensor. These eigenvectors are denoted by $\boldsymbol \xi_i$ and, by assuming that $\mathbf{u}$ is divergence-free, it can be shown that $\boldsymbol \xi_i$ are also divergence-free. Thus, each $\boldsymbol \xi_i$ can be expressed using a potential function $\zeta_i$ via \begin{equation}
    \boldsymbol \xi_i = \nabla^\perp \zeta_i.
    \label{eq:xiGradperp}
\end{equation}
The stochastic term is then introduced to advecting velocity by using the identity \begin{equation}
   \mathbf{u}(t)\text{d}t + \sum_i \boldsymbol\xi_i \circ \text{d}W_t^i = \nabla^\perp \psi(t)\text{d}t + \sum_i \nabla^\perp\zeta_i\circ\text{d}W_t^i.
   \label{eq:stocheqn}
\end{equation}

\paragraph{Numerical implementation.} A full description of the numerical implementation can be found in \cite{cotter2019numerically}, of which only the key details are included here for completeness.\\
A finite element method is employed to solve the system of equations \eqref{eq:hyperboliceqn}, \eqref{eq:gradperpeqn}, and \eqref{eq:poissoneqn}. The Poisson equation for the streamfunction is discretized using a continuous Galerkin scheme, whereas the vorticity equation \eqref{eq:hyperboliceqn} is discretized using a discontinuous Galerkin scheme. The space of discontinuous test functions guarantees numerical conservation of energy in the absence of source terms \cite{bernsen2006dis}. \\
Numerical time integration is performed by applying a third-order strong stability preserving Runge-Kutta (SSPRK3) method. Given a system $q_t = L(q)$, this method reads \begin{equation}
    \begin{aligned}
        q^{(1)} &= q^n + \Delta t L(q^n), \\
        q^{(2)} & = \frac{3}{4}q^{n} + \frac{1}{4}\left[ q^{(1)} + \Delta t L\left(q^{(1)}\right) \right], \\
        q^{n+1} & = \frac{1}{3}q^{n} + \frac{2}{3}\left[ q^{(2)} + \Delta t L\left( q^{(2)}\right) \right].
    \end{aligned}
    \label{eq:SSPRK3}
\end{equation}
Here the superscripts $n$ and $n+1$ denote the $n^\mathrm{th}$ and the ensuing time step, respectively. The internal stages of the Runge-Kutta algorithm are denoted by the superscripts $(1)$ and $(2)$. The time step size is given by $\Delta t$. The time integration scheme for a Stratonovich SPDE is similar. The system given by \begin{equation}
    \text{d}q(t) = L(q(t))\text{d}t + \sum_{i=1}^m G^i(q(t))\circ\text{d}W_t^i
\end{equation}
is integrated via 
\begin{equation}
    \begin{aligned}
        q^{(1)} &= q^n + \Delta t L(q^n) + \sum_{i=1}^n G^i(q^n)\Delta W^i, \\
        q^{(2)} & = \frac{3}{4}q^{n} + \frac{1}{4}\left[ q^{(1)} + \Delta t L\left(q^{(1)}\right) + \sum_{i=1}^n G^i\left(q^{(1)}\right)\Delta W^i \right], \\
        q^{n+1} & = \frac{1}{3}q^{n} + \frac{2}{3}\left[ q^{(2)} + \Delta t L\left( q^{(2)}\right) + \sum_{i=1}^n G^i\left(q^{(2)}\right)\Delta W^i \right].
    \end{aligned}
\end{equation}
Here $\Delta W^i$ denote random samples drawn from a standard normal distribution and multiplied by $\Delta t$.

\paragraph{Deterministic numerical simulation setup.} The deterministic numerical simulation as presented in \cite{cotter2019numerically} is used to generate the EOFs and corresponding time series. The system \eqref{eq:hyperboliceqn}-\eqref{eq:BC} are solved on a grid consisting of $512^2$ computational cells, which will be referred to as the fine grid. A time step size of $\Delta t=0.0025$ is adopted to ensure that a CFL number of $1/3$ is not exceeded. The initial condition of the simulation is described by the vorticity profile \begin{equation}
    \omega = \sin(8\pi x)\sin(8\pi y) + 0.4\cos(6\pi x)\cos(6\pi x) + 0.3\cos(10\pi x)\cos(4\pi y) + 0.02\sin(2\pi y) + 0.02\sin(2\pi x),
\end{equation}
from which the system will reach an equilibrium state after a spin-up time of 100 time units. 


\paragraph{Stochastic numerical simulation setup.} The stochastic numerical simulations are performed on a grid consisting of $64^2$ computational cells, which will be referred to as the coarse grid. A time step size $\Delta t=0.01$ is adopted for each simulation, in accordance with \cite{cotter2019numerically}. The initial conditions are given by the injected fine solution at $t=100$ (after the spin-up time). The fine vorticity is injected on the coarse grid, after which the corresponding streamfunction and velocity fields are calculated.

\paragraph{Perturbation of the initial conditions.} done to see how long the perturbed DNS takes to diverge from the `true' DNS. This gives us a maximum prediction horizon.

\subsection{Data acquisition and processing}
\paragraph{Lagrangian trajectory estimation.} The difference between the Lagrangian trajectories on the fine grid solution and on the filtered fine grid solution provide the measurements that are used in the EOF algorithm. In order to compare the trajectories for the different solutions, we define a fine grid time step $\Delta t_f$ and a coarse grid time step $\Delta t_c = k\Delta t_f$, where $k$ is some integer. Given a fine grid solution $\mathbf{u}^n$ at time $t^n = n\Delta t_c$, the Lagrangian trajectories starting from coordinates $(x_0,y_0)$ are acquired through the following steps.
\begin{itemize}
    \item The solution $\mathbf{u^n}$ is filtered to so that $\bar{\mathbf{u}}^n$ is obtained. The Lagrangian trajectory for the filtered fine grid is estimated via $\Delta t_c \bar{\mathbf{u}}(x_0,y_0)^n$.
    \item An estimate of the true Lagrangian trajectory is found by integrating the movement of a Lagrangian particle over time. That is, we define $(x_{i+1},y_{i+1}) = (x_i,y_i) + \Delta t_f \mathbf{u}(x_i,y_i)$ and apply this step for each of the $k$ fine grid time steps starting from $t^n$. Linear interpolation is applied when the intermediate position of the particle does not coincide with a grid point.
    \item The Lagrangian trajectory corresponding to the filtered solution is subtracted from the estimate of the true trajectory to obtain a distance that `belongs' to the position $(x_0,y_0)$ and time $t^n$.
\end{itemize}
At each coarse grid time step, the initial positions for the particles are chosen as the coarse grid points. The fine grid solution is filtered by applying the Helmholtz operator to the streamfunction $\psi$, i.e., the equation \begin{equation}
    (I-c\Delta)\bar{\psi} = \psi
\end{equation}
is solved for the filtered streamfunction $\bar{\psi}$. Since the coarse grid size consists of 64 cells in each spatial direction, $c$ is chosen equal to $1/64^2$ so that the filtered solution only contains frequencies that are resolvable on the coarse grid.

\paragraph{EOF algorithm and time series computation.} The EOF algorithm decomposes a signal $a(x,t)$ into a time-mean $\xi_0(x)$ and a sum of time series $a_i(t)$ multiplied by eigenfunctions (EOF modes, or EOFs) $\xi_i(x)$ according to \begin{equation}
    a(x,t) = \xi_0(x) + \sum_{i=1}^N a_i(t)\xi_i(x).
\end{equation}
The EOF modes are orthonormal, that is, $\langle \xi_i, \xi_j \rangle = \delta_{ij}$ where $\langle\cdot,\cdot\rangle$ denotes the inner product and $\delta_{ij}$ denotes the Kronecker delta. Due to the orthonormality, the coefficients $a_i(t)$ are readily obtained by taking the inner product of the de-trended measurements with the corresponding EOF mode, \begin{equation}
    a_i(t) = \langle a(x,t)-\xi_0(x), \xi_i(x) \rangle.
\end{equation}

\paragraph{Probability density estimation.} Central to the histogram noise is the assumption that the measured difference in Lagrangian trajectories can be characterized by an underlying probability density. An estimated probability density can then be obtained by constructing a histogram, based on the measurements. The histogram is a statistical estimator and therefore its quality is described by the bias and its robustness under changes of measurements by the variance. A trade-off occurs between these two values. Given a set of measurements, an unbiased histogram can be produced by letting each histogram bin contain only a single measurement, but such an estimator is prone to large changes as more measurements are added. On the other hand, a very robust estimator is obtained by constructing a histogram where all measurements fall within a single bin, although the bias of this histogram would be significant.\\
The number of bins in histogram is of importance, since histograms are determined entirely by the input data and the number of bins. The number of bins adopted here follows from the results presented in \cite{scott2015} and is based on minimizing the asymptotic integrated mean squared error (MSE). The MSE is defined as the sum of the variance and the square of the bias of the histogram. A lower bound for the number of bins is found by minimizing the asymptotic integrated MSE and is given by
 \begin{equation}
\text{Number of bins}\geq \sqrt[3]{2N_M},
\end{equation}
where $N_M$ denotes the number of measurements.

\subsubsection{Random noise generation}
Random numbers are generated using the random sampling package from the NumPy package for Python.
\paragraph{Gaussian noise.} Gaussian noise is generated by sampling from a standard normal distribution and subsequently multiplying by the square root of the time step ($\sqrt{\Delta t}$). The resulting samples are normally distributed with mean zero and variance $\Delta t$.
\paragraph{Histogram noise.}
The histograms are treated as discrete probability distributions. A single bin represents an event, where the height of the bin denotes the probability of that event taking place and the average of the bin edges determine the event value. Samples are drawn from the estimated distribution by applying inverse transform sampling.

\paragraph{Correlated noise.} An Ornstein-Uhlenbeck process is used to generate time-correlated noise. The process is given by the stochastic differential equation \begin{equation}
    \text{d}U(t) = -U(t)\frac{\text{d}t}{T} + \left(\frac{2\sigma^2}{T}\right)^{1/2} \text{d}W(t),
\end{equation}
where $T$ is a (positive) time scale, $\sigma$ is a constant and the initial condition $U(0)\sim\mathcal{N}(0,\sigma^2)$. The notation used here follows from \cite{pope2001}. A discrete form of this equation is given by the autoregressive (AR) model of order 1, \begin{equation}
    \begin{aligned}
        U_i &= U_{i-1} + \text{d}U_i, \\
        \text{d}U_i &= -U_{i-1}\frac{\Delta t}{T} + \left(\frac{2\sigma^2}{T}\right)^{1/2}r_i,
    \end{aligned}
\end{equation}
where $r_i\sim \mathcal{N}(0,\Delta t)$. The value of $T$ is chosen as the decorrelation time of the time series of the EOF modes. The parameter $\sigma$ is set equal to $\sqrt{T/2}$, so that the process reduces to Gaussian noise with variance $\Delta t$ when the decorrelation time is a single time step.\\
The decorrelation time is mode-dependent and is defined as the time at which the autocorrelation attains a nonpositive value for the first time. This way, the decorrelation time measured from the time series of the EOF modes and those of the generated time series using the OU process are similar.



\subsection{Results}
\paragraph{DNS sensitivity study.} Every coarse numerical solution can be regarded as a filtered fine solution. This is not a one-to-one relation, in fact, a filtered solution is invariant under perturbations of the fine solution as long as the perturbed lengthscales are smaller than the coarse grid size. Thus, given a coarse solution one can not know the fine grid solution that corresponds to the former. \\
The initial conditions of the fine simulation are altered by perturbing frequencies that can not be resolved on the coarse grid. By identifying a time at which the perturbed fine simulation results diverge, one identifies the time after which the coarse prediction can no longer be sensibly compared to the DNS result. The idea behind this is that the fine solutions do not correspond to the same filtered (coarse) solution after the fine solutions have diverged.

\paragraph{Temporal correlation of the flow.} To estimate the time scales present in the numerical solution, we compute the inner product of the velocity field at different times. The value \begin{equation}
    \frac{\langle \mathbf{u}(t_i), \mathbf{u}(t_j) \rangle}{\langle\mathbf{u}(t_i), \mathbf{u}(t_i) \rangle} = \frac{\int_\Omega\! \mathbf{u}(t_i) \cdot \mathbf{u}(t_j) \,\text{d}\Omega}{\int_\Omega \! \|\mathbf{u}(t_i)\|^2\text{d}\Omega}
\end{equation}
can be thought of as the similarity between to velocity fields $\mathbf{u}(t_i)$ and $\mathbf{u}(t_j)$. Applying this to the velocity field obtained from the truth and the filtered truth yields an indication of correlation time of the measurements.


\paragraph{Flow measures.}
We can describe the following things (based on the reference paper):\begin{itemize}
    \item Uncertainty quantification plots comparing the truth with the ensemble one standard deviation about the ensemble mean, using point values. We can compare the truth (coarse-grained fine solution), the coarse solution without additional modelling, and the coarse solution with stochasticity. (The 4x4 observation grid is used for data assimilation.) This is useful for comparing the results using a certain type of noise with the true solution. Additionally, plotting the results of multiple types of noise in one plot can be used for comparison between the methods.
    \item The relative $L^2$ distance between the SPDE ensemble and the coarse-grained truth. This quantity is given by \begin{equation}
        d\left(\left\{\hat{q}^i, i=1,\ldots,N_p\right\}\right) = \min_{i\in\{1,\ldots,N_p\}} \frac{\|\omega(t)-\hat{q}^i(t)\|_{L^2(\mathcal{D})}}{\|\omega(t)\|_{L^2(\mathcal{D})}},
    \end{equation}
    which describes the $L^2$ distance of the `best' particle at a given time. (Which particle is the `best' particle can change over time.) This is useful for comparing the results using different types of noise with each other.
\end{itemize}

\paragraph{Measures for predictive capabilities.} Ideas taken from \cite{leutbecher2009diagnosis}, \cite{arnold2013stochastic}, \cite{wilks2011statistical}
\begin{itemize}
    \item Short-term forecasting scale? (see L96 Palmer paper)
    \item rms error - rms spread plots? These plots provide a check for statistical consistency by verifying the relation \begin{equation}
        \frac{M}{M-1}\text{estimate ensemble variance} = \frac{M}{M+1}\text{squared ensemble mean error},
    \end{equation}
    see \cite{arnold2013stochastic}.
\end{itemize}



==> unused.tex <==

\iffalse
\subsection{\label{sec:longtime} Long-time statistics}
In order to understand the long-time effects of the different types of stochastic forcing on the solution, a set of time-averaged quantities are studied. The averages are obtained by sampling the numerical solution at every time unit after the spin-up time, for a total of 365 time units. A single realization is considered for each type of stochastic forcing.\\
\textbf{\textit{Remove figure b}}

\textit{Perhaps something like pdfs of the vorticity at certain points in the domain could be interesting as well?}

\begin{figure}[h!]
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    \includegraphics[width=\textwidth]{figures_general/average_vorticity_spectra.eps}
    \caption{Average energy spectra of cross-sections of the vorticity field in $x$-direction.}
    \label{fig:RMSRME_filtered_DNS}
    \end{subfigure}
    \begin{subfigure}[t]{0.45\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures_general/average_fluctuation_spectra.eps}
    \caption{Average energy spectra of cross-sections of the vorticity fluctuation field in $x$-direction.}
    \label{fig:RMSRME_coarse_with_xis}
    \end{subfigure}
    \caption{Test caption}
\end{figure}
\fi
